Testing Assignments to Constraint Satisfaction Problems

For a finite relational structure A, let CSP(A) denote the CSP instances whose constraint relations are taken from A. The resulting family of problems CSP(A) has been considered heavily in a variety of computational contexts. In this article, we consider this family from the perspective of property testing: given an instance of a CSP and query access to an assignment, one wants to decide whether the assignment satisfies the instance, or is far from so doing. While previous works on this scenario studied concrete templates or restricted classes of structures, this article presents comprehensive classification theorems. Our first contribution is a dichotomy theorem completely characterizing the structures A such that CSP(A) is constant-query testable: (i) If A has a majority polymorphism and a Maltsev polymorphism, then CSP(A) is constant-query testable with one-sided error. (ii) Else, testing CSP(A) requires a super-constant number of queries. Let $\exists$CSP(A) denote the extension of CSP(A) to instances which may include existentially quantified variables. Our second contribution is to classify all structures A in terms of the number of queries needed to test assignments to instances of $\exists$CSP(A), with one-sided error. More specifically, we show the following trichotomy: (i) If A has a majority polymorphism and a Maltsev polymorphism, then $\exists$CSP(A) is constant-query testable with one-sided error. (ii) Else, if A has a $(k + 1)$-ary near-unanimity polymorphism for some $k \geq 2$, and no Maltsev polymorphism then $\exists$CSP(A) is not constant-query testable (even with two-sided error) but is sublinear-query testable with one-sided error. (iii) Else, testing $\exists$CSP(A) with one-sided error requires a linear number of queries.

==> monotone-circuit.tex <==
%!TEX root=main.tex

\subsection{Monotone circuits that are hard to test with one-sided error}
In this section, we show the following.
\begin{theorem}\label{the:hard-monotone-circuits}
  For any $\eta >0 $ and infinitely many $n \in \bbN$,
  there exists a monotone circuit $C_{n,\eta}$ with the following property:
  \begin{itemize}
  \item The number of $\vee$-gates in $C_{n,\eta}$ is $O(n^{1+\eta})$.
  \item Any one-sided error tester for $C_{n,\eta}$ requires $\Omega(n)$ queries.
  \end{itemize}
\end{theorem}

For odd $n \in \bbN$, let $\Maj_n$ be the majority function over $n$ variables.
For $n \in \bbN$ and $0 \leq k \leq n$, let $\Th_n^k$ be the threshold function on $n$ variables, that is, $\Th_n^k(x_1,\ldots,x_n) = 1$ if and only if $\sum_{i \in [n]}x_i \geq k$.
We can construct $\Maj_n$ using a polynomial number of $\vee$-gates:
\begin{lemma}\label{lem:vee-gatesin-majority}
  Let $n \in \bbN$ be odd.
  Then, we can construct $\Maj_n$ as a monotone circuit using at most $O(n^3)$ $\vee$-gates.
\end{lemma}
\begin{proof}
  Note that $\Maj_n = \Th_n^{\ceil{n/2}}$.
  We use the following recursive construction of $\Th_n^k$.
  \begin{align*}
    \Th_n^0(x_1) & = 1,   \\
    \Th_n^1(x_1) & = x_1, \\
    \Th_n^k(x_1,\ldots,x_n) & = \bigvee_{\ell \leq \min\set{k,\floor{n/2}}} \Bigl(\Th_n^\ell(x_1,\ldots,x_{\floor{n/2}}) \wedge \Th_n^{k-\ell}(x_{\floor{n/2}+1},\ldots,x_n)\Bigr) & (n \geq 2).
  \end{align*}
  The number of $\vee$-gates used to construct $\Maj_n$ is at most $\sum_{n' \in [n]} \sum_{0 \leq k \leq n'} (k-1) = O(n^3)$.
\end{proof}

For $c \in \bbN$ and $n$ such that $n^{1/c}$ is an odd integer, we define $\RMaj_{n,c}$ as the circuit represented by a complete $n^{1/c}$-ary tree of depth $c$, where each internal node corresponds to a $\Maj_{n^{1/c}}$-circuit and each leaf is associated with a unique variable.
Note that the number of variables of $\RMaj_{n,c}$ is exactly $n$.
We now show that $\RMaj_{n,c}$ achieves Theorem~\ref{the:hard-monotone-circuits} for an appropriate choice of $c$.
\begin{proof}[Proof of Theorem~\ref{the:hard-monotone-circuits}]
  We assume $n$ is sufficiently large and choose $c$ so that $\eta = 2/c$.

  The number of $\Maj_{n^{1/c}}$-circuits in an $\RMaj_{n,c}$-circuit is $\sum_{0 \leq k \leq c-1} n^{k/c} = O(n^{(c-1)/c})$.
  Since each $\Maj_{n^{1/c}}$-circuit uses $n^{3/c}$ $\vee$-gates from Lemma~\ref{lem:vee-gatesin-majority}, the total number of $\vee$-gates is $O(n^{(c-1)/c} \cdot n^{3/c}) = O(n^{(c+2)/c}) = O(n^{1+\eta})$.

  We now show that $\RMaj_{n,c}$ is a hard circuit for one-sided error testers.

  To this end, we first show that a $\Omega(1/2^c)$-fraction of variables should be assigned one to make $\RMaj_{n,c}$ evaluate to one.
  In order to make the majority circuit in the top level evaluate to one, at least $\floor{n^{1/c}/2}$  majority circuits in the second level must evaluate to one.
  In order to make these majority circuits evaluate to one, at least $(\floor{n^{1/c}/2})^2$  majority circuits in the third level must evaluate to one, and so on.
  In total, in order to make $\RMaj_{n,c}$ evaluate to one, the number of variables assigned one must be at least $(\floor{n^{1/c}/2})^{c} = (n^{1/c}-1)^c/2^{c} > n/2^{c+1} =: \epsilon n$.

  Next, we show that a $\Omega(1/2^c)$-fraction of variables should be assigned zero to make $\RMaj_{n,c}$ evaluate to zero.
  To see this, we can use a similar argument as before.
  In order to make the majority circuit in the top level evaluate to zero, at least $\floor{n^{1/c}/2}$  majority circuits in the second level must evaluate to zero.
  In order to make these majority circuits evaluate to zero, at least $(\floor{n^{1/c}/2})^2$  majority circuits in the third level must evaluate to zero, and so on.
  In total, in order to make $\RMaj_{n,c}$ evaluate to zero, the number of variables assigned zero must be at least $(\floor{n^{1/c}/2})^{c} = \epsilon n$.

  Now consider a one-sided error tester for $\RMaj_{n,c}$ that queries at most $\epsilon n /2$ variables.
  Let $\set{x_i}_{i \in S}$ be the set of variables that the tester has queried.
  Since $|S| < \epsilon n$, the output of $\RMaj_{n,c}$ becomes one by setting $x_i = 1$ for all $[n] \setminus S$.
  Hence, the tester cannot reject because it is a one-sided error tester.
  However, since $|S| < \epsilon n/2$, the assignment obtained by setting $x_i = 0$ for all $[n] \setminus 0$ is $\epsilon/2$-far from satisfying assignments.
  Hence, any one-sided error tester cannot distinguish satisfying assignments from $\epsilon/2$-far assignments with $\epsilon n/2$ queries.
\end{proof}


